On the Hardness of Gray Code Problems for Combinatorial Objects

Can a list of binary strings be ordered so that consecutive strings differ in a single bit? Can a list of permutations be ordered so that consecutive permutations differ by a swap? Can a list of non-crossing set partitions be ordered so that consecutive partitions differ by refinement? These are examples of Gray coding problems: Can a list of combinatorial objects (of a particular type and size) be ordered so that consecutive objects differ by a flip (of a particular type)? For example, 000, 001, 010, 100 is a no instance of the first question, while 1234, 1324, 1243 is a yes instance of the second question due to the order 1243, 1234, 1324. We prove that a variety of Gray coding problems are NP-complete using a new tool we call a Gray code reduction.

==> lipics-v2019-authors/CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file


==> temp.tex <==
This file is used for converting Google Doc material to LaTeX.

%%%%%%%%%%

Consider an arbitrary instance of the source problem, $\HPGrid{P}$, where $P$ is in standard position and has $k$ points.  
Let $c-1$ and $r-1$ be the maximum $x$ and $y$ values in $P$, respectively.  
In other words, $P$ spans $r$ rows and $c$ columns of the infinite grid.

First we check if the grid graph $G[P]$ is connected.
If not, we immediately answer no, since $G[P]$ cannot have a Hamilton path.
This pre-processing step can be done in polynomial-time with respect to the size of the input, so it is ``free'' with respect to our polynomial-time reduction.
A consequence of this step is that we may assume that $k \geq r$ and $k \geq c$, since $G[P]$ is disconnected if there are any empty rows and columns.
This assumption will be helpful when we justify that our reduction runs in polynomial-time.

We construct a subset of binary strings $S \subseteq \BINARY{m}$ with $m = (r-1) + (c-1)$.
The size of the subset is $|S| = k$, with each point in $P$ contributing one string to the subset.
Each string consists of a prefix of length $r-1$ which is based on the point's row, followed by a suffix of length $c-1$ which is based on the point's column.
More specifically, the rows and columns are using string from $R$ and $C$ below, respectively, 
\begin{align} \label{eq:encodePrefixSuffix}
A = \{0^{r-1}, 10^{r-2}, 110^{r-3}, \ldots, 1^{r-1}\} && B = \{0^{c-1}, 0^{c-2}1, 0^{c-3}11, \ldots, 1^{c-1}\}
\end{align}
where exponentiation denotes concatenation.
Precisely, the set $S$ is defined below.
\begin{equation*}
S = \{ 1^x 0^{r-x-1} 0^y 1^{c-y-1}   |  (x, y) \in P \}
\end{equation*}
We say that the string $\blue{1^x 0^{r-x-1}}  \red{0^{c-y-1} 1^y}  \in S$ corresponds to the point $(x, y) \in P$, and vice versa.  
Now we prove that $\HPGrid{P}$ and $\GrayD{S}$ have the same answer.

Suppose that $\HPGrid{P}$ is yes.  
Therefore, $G[P]$ has a Hamilton path.  
Let $H = (x_1, y_1), (x_2, y_2), \ldots, (x_k, y_k)$ be an order of the points in a Hamilton path.  
Let $C$ be the corresponding order of strings in $S$.  
We claim that $C$ is a Gray code.  
To prove this, we start by noting that in $H$, each consecutive pair of points $(x, y), (x', y')$ differ by one in either the $x$ or $y$ coordinate.  
In the former case, we know that $x' \in \{x-1, x+1\}$ and $y' = y$.  
Therefore, there are only two possibilities for the consecutive pair of corresponding binary strings:
\begin{itemize}
    \item $\blue{1^x 0^{r-x-1}}  \red{0^{c-y-1} 1^y}$ is followed by $\blue{1^{x-1} 0^{r-x}}  \red{0^{c-y-1} 1^y}$, or
    \item $\blue{1^x 0^{r-x-1}}  \red{0^{c-y-1} 1^y}$ is followed by $\blue{1^{x+1} 0^{r-x-2}}  \red{0^{c-y-1} 1^y}$.
\end{itemize}
In both cases, this is a valid Gray code change, since only a single bit is modified.  
A similar argument handles the case in which the y coordinate differs.
Therefore, $C$ is a Gray code.

Suppose that $\GrayD{S}$ is yes.  
Therefore, $S$ has a Gray code $C = b_1, b_2, \ldots, b_k$.  
Let $H$ be the corresponding order of points in $P$.  
We claim that $H$ is an order of points on a Hamilton path in $G[P]$.  
Consider a consecutive pair of strings, $b_{i} = \blue{\alpha} \red{\beta}$ and $b_{i+1} = \blue{\alpha'} \red{\beta'}$, where $|\red{\alpha}| = |\red{\alpha'}| = r-1$ and $|\blue{\beta}| = |\blue{\beta'}| = c-1$.
Only a single bit changes between $b_{i}$ and $b_{i+1}$, so either $\blue{\alpha} = \blue{alpha'}$ and $\red{\beta} \noteq \red{\beta'}$, or $\blue{\alpha} \neq \blue{alpha'}$ and $\red{\beta} = \red{\beta'}$.  
Let us consider the former case.  
In this case, we also know that only a single bit changes between $\red{\beta}$ and $\red{\beta'}$.  Furthermore, based on the suffix set $B$ from \eqref{eq:encodePrefixSuffix}, there are two possibilities for the pair of corresponding points:
\begin{itemize}
    \item $(x, y)$ is followed by $(x', y')$ where $x' = x - 1$ and $y' = y$ (i.e. a move to the left), or
    \item $(x, y)$ is followed by $(x', y')$ where $x' = x + 1$ and $y' = y$ (i.e. a move to the right).
\end{itemize}
In both cases, $(x, y)$ and $(x', y')$ are adjacent in $G[P]$.  
A similar argument handles the case when the prefix changes, with the two possibilities translating to up and down moves in the graph.  
Therefore, $H$ is an order of points around a Hamilton path.


==> unused/AaronOld.tex <==

\section{Aaron's notes to discuss}
\label{sec:discuss}


Re: permutations.
By doing a direct grid graph reduction, we can show that the subset Gray code problem is hard for permutations and swaps, even when limited to permutations whose only inversions involve 1 or n.
(This was in an older version of the abstract)

Re: outline.
The selection of results is not meant to be exhaustive.
It is also important to note that hypercube reductions cannot be applied in all situations since some flip graphs do not contain induced hypercubes of sufficient size.
Furthermore, some Gray code problems can be solved in polynomial-time (e.g., those related to de Bruijn sequences and shorthand universal cycles).
On the other hand, our results do comprise a surprisingly rich swatch of combinatorial objects and operations.
These topics are discussed further in Section \ref{sec:final}.

Re: generalization versus specialization for objects.
when establishing Gray codes want to consider more general objects.
example of strengthening combinations or permutations to multiset permutations, or from binary to $k$-ary.
when establishing hardness want to consider more specific objects.
example of strengthening hardness from multiset permutations to combinations or permutations, or from $k$-ary to binary.
for this reason, readers should expect to see the simplest objects studied here, and know that they apply to more general objects.

Re: generalization versus specialization for operations.
generalization and specialization becomes more subtle when we shift from objects to operations.
generalizing the set of operations can change a difficult problem to an easy problem.
for example, consider an overpowered generalization of bit-flips which allows any subset of bits to be complicated.
in this case, the Gray code problem is easy to solve as the answer is always yes, since any pair of $n$-bit strings differ by one application of this overpowered operation.
on the other hand, one could consider the underpowered set of operations that only allows the first bit to be complicated.
in this case, the Gray code problem is easy to solve as the answer is always no, except when there is a single string or two strings differing only in the first bit.
thus, changes in the operation set are not monotonic with respect to generalization.
for this reason, readers should expect to see a variety of operations studied here, such as various types of transpositions including adjacent, homogeneous, and unrestricted.
mention exception and possibly put it in a remark.



Here we strengthen some of our results to operation subsets...

Aaron: perhaps we want some general statements like the following
\begin{itemize}
    \item If a problem is hard for $\objSet{O}$ and $\flipSet{F}$, then it is still hard for an object superset $\objSet{O'} \supseteq \objSet{O}$ so long as the operations do not change for $\objSet{O}$.
    For example, $k$-ary Gray codes are hard because bit flip Gray codes are hard, so long as the operations for $k$-ary Gray codes allow $0$s to be changed to $1$s and vice versa.
    (This consequence would not be immediate if we considered $k$-ary Gray codes in which each symbol can only be incremented mod $k$.)
\end{itemize}


==> unused/abstractOld.tex <==
%%% See outtakes.tex for other older abstracts


\begin{abstract}
It is well-known that \textsc{HamiltonPath} is NP-complete for grid graphs.
Stated another way, \textsc{HamiltonPath} is NP-complete for the induced subgraphs of rectangular grid graphs.
This leads to a natural question:
Is \textsc{HamiltonPath} hard for the induced subgraphs of other graph families?
Similarly, \textsc{Domination} and  is NP-complete for a given subset of $n$-bit binary strings.
Stated another way, \textsc{CoveringRadius} is NP-complete for the induced subgraphs of the $n$-dimensional hypercube.
Is the problem hard for other underlying graph families?
Likewise, \textsc{Domination} is NP-complete for the induced subgraphs of the associahedron.
Is this true for other graph families?

Yes answers to these questions can be established by efficiently finding induced subgraphs of a new graph family that are isomorphic to the graph family for which the problem is known to be hard.
then take it to the next step by finding induced in those ...
% For example, if we can find an $n$-dimensional hypercube as an induced subgraph of an $m$-dimensional permutohedron, and efficiently map form the former's vertices to the latter's vertices, then the covering radius problem is NP-complete for the induced subgraphs of the permutohedron.
This begs for the existence of a simple and systematic approach to determining which graph families are induced subgraphs of other graph families, and to develop efficient maps between their vertices.
This paper aims to be such a resource.
In particular, provide \emph{polynomial-time induced subgraph reductions} for dozens of natural graph families.

% In this paper, we show that the answer to these questions, and many others, is yes, for dozens of natural families of graphs.

% Each result is obtained by a relatively simple \emph{polynomial-time induced subgraph reduction} from grid graphs, hypercubes, or permutohedron. 

% Consequences of our results include the sharpening of various NP-hardness results for graphs, and the NP-hardness for a wide variety of subset Gray code problems.
% For example, \textsc{Domination} is NP-complete when restricted to permuticals (i.e., induced subgraphs of the permutohedron), and it is NP-complete to decide if a subset of $n$-bit binary strings has a Gray code ordering (i.e., consecutive strings differ in one bit).

Namrata : add associahedron and covering code problems (https://link.springer.com/article/10.1007/bf02679443)
\end{abstract}


\begin{abstract}
It is well-known that \textsc{HamiltonPath} is NP-complete for grid graphs.
Stated another way, \textsc{HamiltonPath} is NP-complete for the induced subgraphs of rectangular grid graphs.
This leads to a natural question:
% Is \textsc{HamiltonPath} NP-complete when restricted to the subgraphs of other families of graphs?
% Are there other families of graphs for which subgraph Hamiltonicity problems are NP-complete?
Is \textsc{HamiltonPath} hard for the induced subgraphs of other graph families?
Similarly, \textsc{CoveringRadius} is NP-complete for a given subset of $n$-bit binary strings.
Stated another way, \textsc{CoveringRadius} is NP-complete for the induced subgraphs of the $n$-dimensional hypercube.
Is the problem hard for other underlying graph families?
Likewise, \textsc{Domination} is NP-complete for the induced subgraphs of the associahedron.
Is this true for other graph families?

Yes answers to these questions can be established by efficiently finding induced subgraphs of a new graph family that are isomorphic to the graph family for which the problem is known to be hard.
% For example, if we can find an $n$-dimensional hypercube as an induced subgraph of an $m$-dimensional permutohedron, and efficiently map form the former's vertices to the latter's vertices, then the covering radius problem is NP-complete for the induced subgraphs of the permutohedron.
This begs for the existence of a simple and systematic approach to determining which graph families are induced subgraphs of other graph families, and to develop efficient maps between their vertices.
This paper aims to be such a resource.
In particular, provide \emph{polynomial-time induced subgraph reductions} for dozens of natural graph families.

% In this paper, we show that the answer to these questions, and many others, is yes, for dozens of natural families of graphs.

% Each result is obtained by a relatively simple \emph{polynomial-time induced subgraph reduction} from grid graphs, hypercubes, or permutohedron. 

% Consequences of our results include the sharpening of various NP-hardness results for graphs, and the NP-hardness for a wide variety of subset Gray code problems.
% For example, \textsc{Domination} is NP-complete when restricted to permuticals (i.e., induced subgraphs of the permutohedron), and it is NP-complete to decide if a subset of $n$-bit binary strings has a Gray code ordering (i.e., consecutive strings differ in one bit).

Namrata : add associahedron and covering code problems (https://link.springer.com/article/10.1007/bf02679443)
\end{abstract}



\begin{abstract}
Consider the following decision problem where $\BINARY{n}$ is the set of $n$-bit binary strings:
Can a set $S \subseteq \BINARY{n}$ ordered such that consecutive strings differ in a single bit?
In other words, is there a Hamilton path in the induced subgraph $\CubeGraph{n}[S]$, where $\CubeGraph{n}$ is the $n$-cube with vertex set $\BINARY{n}$?
Famously, the answer is yes when $S = \BINARY{n}$ by the binary reflected Gray code, and when $S = \COMBOS{2k+1}{k}$ by Mütze's middle levels theorem.
We prove that the general question is NP-complete.
% In other words, it is NP-complete to determine if an arbitrary induced subgraph of the $n$-cube has a Hamilton path.
In fact, this holds even when the strings (or induced vertices) are restricted to peakless strings of the form $1^* 0^* 1^*$.
[This is already in the Rubik's hypercube paper! \cite{demaine2018solving}]

Using this new result, we prove that a wide variety of \emph{subset Gray code} problems are NP-complete.
For example, it is NP-complete to determine if a set of permutations can be ordered by adjacent-transpositions, or equivalently, if induced subgraphs of the permutahedron $\PermGraph{n}$ have Hamilton paths.
% In fact, this is true even when the inversions are restricted to the symbols $1$ and $n$. 
We obtain this result by showing that $\PermGraph{2n}$ has $\CubeGraph{n}$ as an induced subgraph, and we refer to this general argument as a \emph{hypercube reduction}.
The effectiveness of this technique is far reaching, as we find large hypercubes (as well as grids and permutohedron) as induced subgraphs in a wide variety of flip graphs involving trees, matchings, diagonalizations, rectangulations, and many more.
%(i.e., binary, ordered, spanning)
% For example, the problem is NP-complete for spanning trees of a graph using edge swaps, and for binary trees using the rotation operation.
Collectively, these new hardness results provide a complexity backdrop for a wide variety of papers in the area of combinatorial generation.
\end{abstract}
\end{abstract}

==> unused/backgroundOld.tex <==
%%% Our original section on background material
%%% This includes some definitions and notation that we may need

\section{Background}
\label{sec:back}

This section includes background material.

\subsection{Objects and Flips}
\label{sec:back_objects}

% Aaron: If we want our decision problems to be in NP, then we need to be able to apply the operations in polynomial-time.
% Otherwise, we can't efficiently verify a certificate (i.e., verify that a provided Hamilton path in the flip graph is indeed a Hamilton path) because we can't efficiently verify if two vertices are connected by an edge, and so we can't claim membership in NP.
% Perhaps the best way of proceeding is to bake polynomial-time into our definition of an \emph{operation}.
% Here polynomial-time should be related to the size of an individual object.
% We'll also want to say that the size of all of the objects are polynomially related, otherwise the previous convention gets messy.
% But we can only do theabove when we talk about families of objects and operations.
% So we'll need to be very careful in our definition of a flip graph.

We use the term \emph{objects} to refer to sets of all combinatorial objects of a particular type parameterized by size.
For example, $\BINARY{n}$ is the set of $n$-bit binary strings, and $\GRAPHS{n}$ is the set of simple undirected graphs with $n$ vertices.
For convenience, we assume that every object of the same size is encoded using the same number of bits.
This is obviously true for $\BINARY{n}$ and for $\GRAPHS{n}$ encoded as adjacent matrices;
if adjacency lists are used, then the complete graph $\graph{K_n} \in \GRAPHS{n}$ provides the encoding size of each graph.

We use the term \emph{flips} to refer to sets of operations that can be applied to objects. % again parameterized by size.
For example, $\BITFLIPS{n} = \{\bitFlip{1}, \bitFlip{2}, \ldots, \bitFlip{n}\}$ is the set of bit flip operations, where $\bitFlip{i} : \BINARY{n} \rightarrow \BINARY{n}$ complements the $i$th bit of $b_1 b_2 \ldots b_n \in \BINARY{n}$.
We only consider flips with the following \emph{efficiency property}:
Given objects $x, y \in \objSet{O}$, we can determine if there exists a flip $f \in \flipSet{F}$ with $f(x) = y$ in polynomial-time with respect to the encoding size of $x$ (or equivalently, $y$).
Operations can also depend on the specific object.
For example, if the objects are perfect matchings of a particular graph $\graph{G}$, then the alternating cycles that can be flipped depend on the specific perfect matching%
\footnote{Note that alternating cycle flips have the efficiency property.
This is because perfect matchings differ by such a flip, if and only if, their exclusive-or form a cycle in the graph $\graph{G}$.}.

\subsection{Flip Graphs}
\label{sec:back_flipgraph}

The \emph{flip graph} for objects $\objSet{O}$ and flips $\flipSet{F}$ has vertex set $\objSet{O}$, edges based on $\flipSet{F}$, and is denoted $\flipGraph{\objSet{O}}{\flipSet{F}}$.
For example, if the objects are binary strings (i.e., $\objSet{O} = \BINARY{n}$) and the flips are bit-flips (i.e., $\flipSet{F} = \BITFLIPS{n}$), then the flip graph is ...  be the set of all $n$-bit binary strings.
We index the bits in a binary string from left-to-right starting at index $1$, so if $b \in \BINARY{n}$, then $b = b_1 b_2 \cdots b_n$.
The \emph{$n$-dimensional hypercube} (or simply, \emph{$n$-cube}) $\CubeGraph{n}$ has vertex set $\BINARY{n}$ and edges between vertices that differ in a single bit.
In other words, $\CubeGraph{n}$ is the flip graph $\flipGraph{\BINARY{n}}{\flipSet{F}}$, where $\BITFLIPS{n}$ is the set of operations $\bitFlip{i} : \BINARY{n} \rightarrow \BINARY{n}$ that flips the $i$th bit for $1 \leq i \leq n$.
See Figure \ref{fig:hypercube}.

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.325\textwidth}
        \centering 
        \includegraphics{hypercube2}
        \caption{Hypercube $\CubeGraph{2}$.}
        \label{fig:hypercube_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.325\textwidth}
        \centering 
        \includegraphics{hypercube3}
        \caption{Hypercube $\CubeGraph{3}$.}
        \label{fig:hypercube_3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.325\textwidth}
        \centering 
        \includegraphics{hypercubeSubgraph3}
        \caption{Induced subgraph $\CubeGraph{3}[S]$ for $S = \{000, 001, 011, 100, 101, 111\}$.
        todo: create one that has a path but not a cycle}
        \label{fig:hypercube_subgraph3}
    \end{subfigure}
    \caption{The hypercube $\CubeGraph{n}$'s vertices are the $n$-bit binary strings $\BINARY{n}$ with edges corresponding to individual bit flips.
    In other words, $\CubeGraph{n}$ is the flip graph $\flipGraph{\BINARY{n}}{\BITFLIPS{n}}$.
    Determining if an arbitrary induced subgraph has a Hamilton path or cycle is NP-complete.}
    \label{fig:hypercube}
\end{figure}

\subsection{Gray Code Problems / Induced Subgraph Hamilton Path Problems}
\label{sec:back_gray}

Here we define our general problem and prove that it is in NP.

\begin{definition} \label{def:GrayDP}
Let $\objSet{O}$ be a set of objects, and $\flipSet{F}$ be a set of operations that operate on the objects (i.e., $f : \objSet{O} \rightarrow \objSet{O}$ for all $f \in \flipSet{F}$).
The decision problem $\GrayI[\objSet{O},\flipSet{F}]{S}$ asks if a given subset of objects $S \subseteq \objSet{O}$ can be given a total order, 
\begin{equation*}
s_1, s_2, \ldots, s_m \text{ where } m = |S|
\end{equation*}
such that for all $1 \leq i < m$, 
\begin{equation*}
s_{i+1} = f(s_{i}) \text{ for some } f \in \flipSet{F}.    
\end{equation*}
In other words, the answer is yes if the object subset can be sequenced so that each object is transformed into the next by applying one of the operations.
We refer to $\GrayDP{\objSet{O},\flipSet{F}}$ as the \emph{Gray code problem on $\objSet{O}$ using $\flipSet{F}$}.
\end{definition}

Let $\HPATH{\graph{G}}$ be the decision problem of whether graph $\graph{G}$ has a Hamilton path.
The Gray code decision problem is equivalent to asking if the flip graph $\flipGraph{\objSet{O}}{\flipSet{F}}$ has an Hamilton path when induced on $S$.
That is, $\GrayI[\objSet{O},\flipSet{F}]{S} = \HPATH{\flipGraph{\objSet{O}}{\flipSet{F}}[S]}$.
We refer to the latter as a \emph{induced subgraph Hamilton path problem}.

Note that the Gray code problem $\GrayI[\objSet{O},\flipSet{F}]{S}$ is equivalent to asking if the associated flip graph has a Hamilton path when induced on the subset of objects (i.e., vertices) $S \subseteq \objSet{O}$.
When the context is clear, we'll omit the objects and operations and write $\GrayI{S}$ instead of $\GrayI[\objSet{O},\flipSet{F}]{S}$.

\begin{lemma} \label{lem:NP}
The Gray code problem $\GrayDP{\objSet{O},\flipSet{F}}$ (or equivalently, the corresponding induced subgraph Hamilton path problem $\HPATH{\flipGraph{\objSet{O}}{\flipSet{F}}[S]}$) is in NP.
\end{lemma}
\begin{proof}[Lemma \ref{lem:NP}]
Consider the underlying flip graph $\graph{G} = \flipGraph{\objSet{O}}{\flipSet{F}}$.
Recall that our operations can be evaluated in polynomial-time.
More specifically, if $u,v \in \objSet{O}$, then we can test if $v = f(u)$ for some $f \in \flipSet{F}$ in polynomial-time relative to the size of an object in $\objSet{O}$.
In other words, we can determine if $(u,v)$ is an edge in polynomial-time.
Hence, a suitable certificate is a list of objects (or equivalently, vertices) and our verification algorithm checks if the list contains each member of $S$ exactly once, and that consecutive members are connected by an edge.
% relative to the input size of $S$ 
\end{proof}

todo: cycle variants $\HCYCLE{G}$?

\subsection{Grid Graphs and Hamiltonicity}
\label{sec:back_grid}

It is well-known that the decision problem $\HPATH{G}$ is strongly NP-complete.
The result is also true when restricted to grid graphs.

More formally, a \emph{grid graph} is ...
Note that the term grid graph refers induced subraphs and not arbitrary subgraphs ...
The \emph{grid graph Hamilton path problem $\HPGrid{P}$} asks if a grid graph $G[P]$ has a Hamilton path, and it is illustrated in Figure \ref{fig:HPGrid}.
It is known to be strongly NP-complete \cite{itai1982hamilton}.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.46\textwidth}
        \centering 
        \includegraphics[scale=0.35]{GridGraphPoints}
        \caption{$P = \{(0,0), \ldots, (7,2)\}$ in standard position.}
        \label{fig:HPGrid_points}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering 
        \includegraphics[scale=0.35]{GridGraph}
        \caption{The grid graph $G[P]$.}
        \label{fig:HPGrid_graph}
    \end{subfigure}
    \begin{subfigure}[b]{0.27\textwidth}
        \centering 
        \includegraphics[scale=0.35]{GridGraphPath}
        \caption{A Hamilton path in $G[P]$.}
        \label{fig:HPGrid_path}
    \end{subfigure}
    \caption{Illustrating a yes instance of the $\HPGrid{P}$ decision problem.}
    \label{fig:HPGrid}
\end{figure}

Aaron: We need to discuss how $\HPGrid{G}$ problems are encoded.


==> unused/basegraphs.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[scale=1.0]{graphs/grid3by3}
        \caption{The rectangular grid graph $\GridGraph{3}{3}$.}
        \label{fig:baseGraphs_grid}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[scale=1.0]{graphs/hypercube3.pdf}
        \caption{The hypercube $\CubeGraph{3}$.}
        \label{fig:baseGraphs_cube}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[scale=1.0]{permutohedron3}
        \caption{The permutohedron $\PermGraph{3}$.}
        \label{fig:baseGraphs_permutohedron}
    \end{subfigure}
    \caption{Instances of three well-known graphs.
    Lemma \ref{lem:induces} shows that $\GridGraph{r}{c}$ is an induced subgraph of $\CubeGraph{2n-2}$ where $n=r+c$,
    and $\CubeGraph{n}$ is an induced subgraph of $\PermGraph{2n}$.
    For the next larger permutohedron $\PermGraph{4}$ see Figure \ref{fig:permutohedron4}.
    }
    \label{fig:baseGraphs}
\end{figure}



\begin{figure}[h]
    \centering
    \begin{tabular}{r|c|c|c|} \cline{2-4}
     graph family & rectangular grid graphs $\GridGraph{r}{c}$ & hypercube graphs $\CubeGraph{n}$ & permutohedron $\PermGraph{n}$  \\
     induced subgraphs & grid graphs & cubical & permutical  \\ \cline{2-4}
    \end{tabular}
    \caption{Names of three graph families and their induced subgraphs.
    The name \emph{permutical} is new.
    Aaron: this table should be removed ... the term cubical is used in multiple ways in the literature and we are no longer focusing on permutohedron.}
    \label{fig:names}
\end{figure}


==> unused/binaryOld.tex <==
\section{Problems on Binary Strings}
\label{sec:binary}

In this section we consider additional problems involving binary strings.
First we'll strengthen our initial hardness result involving bit flips.
Then we'll prove a new result involving a more general operation of substring complements.
The second result will demonstrate the hypercube reduction strategy.

\subsection{Bit Flips on Peakless Binary Strings}
\label{sec:binary_flips}

Let $\bitFlip{i}$ be the operation of flipping the $i$th bit and $\BITFLIPS{n} = \{\bitFlip{1}, \bitFlip{1}, \ldots, \bitFlip{1}\}$ be the set of all flips that can act on strings in $\BINARY{n}$.
For example, $\bitFlip{3}(0000) = 0010$.

A \emph{peak} in a binary string is a substring of the form $0 1^+ 0$.
A binary string is \emph{peakless} if it contains no peaks.
Let $\PEAKLESS{n} \subseteq \BINARY{n}$ be the set of $n$-bit peakless strings.
We can strengthen Lemma \ref{lem:induces} by noting that the reduction only creates peakless binary strings.

\begin{corollary} \label{cor:peakless}
The decision problem $\GrayDecision{\PEAKLESS{n}}{\BITFLIPS{n}}$ is strongly NP-complete.
%, where $\PEAKLESS{n} \subseteq \BINARY{n}$ is the set of peakless $n$-bit binary strings.
\end{corollary}



\subsection{Substring Complements}
\label{sec:binary_subs}

Let $\bitSub{i}{j}$ the the operation of flipping every bit in the substring of bits $i$ through $j$ for $i \leq j$.
Let $\COMPS{n}$ be the set of all such operations.
We let $\CompGraph{3}$ denote the associated \emph{substring complement graph}, which is the flip graph.
In general, $\CompGraph{n}$ is the flip graph $\flipGraph{\BINARY{n}}{\COMPS{n}}$.    

The next decision problem that we consider is $\GrayDecision{\BINARY{n}}{\COMPS{n}}$.

Note that this \emph{substring complement} operations include the individual bit flips from Section \ref{sec:binary_flips} as $\bitSub{i}{i} = \bitFlip{i}$.
Thus, if we want to prove that $\GrayDecision{\BINARY{n}}{\COMPS{n}}$  is hard, then it must be that the greater operational flexibility doesn't make the problem tractable.
In other words, the extra edges in $\CompGraph{n}$ (relative to $\CubeGraph{n}$) do not make it easier to determine if subgraphs have Hamilton paths.
Note: If we were to further generalize the operation set to allow any set of bits to be complemented, then the problem would be easy, since any string could be followed by any other string.

The hypercube reduction strategy requires us to find $n$-cubes $\CubeGraph{n}$ as induced subgraphs within $\CompGraph{m}$, and for $m$ to be polynomially bounded with respect to $n$.
This is accomplished by using `padding' in Theorem \ref{thm:binary} and is illustrated in Figure \ref{fig:binary_complements}.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\textwidth]{binaryComplementCube3}
        \caption{Binary strings of the form $\bits{b_1} \padding{1} \bits{b_2} \padding{1} \ldots \padding{1} \bits{b_n}$ from \eqref{eq:binaryComplement} with substring complements.}
        \label{fig:binary_complements}
    \end{subfigure}
    \hfill
    \caption{
    Hypercube reduction that establish NP-hardness for Gray code problems involving binary strings and substring complements.
    }
    \label{fig:binary}
\end{figure}

\begin{theorem} \label{thm:binary}
Gray code problems are NP-hard for binary strings $\BINARY{n}$ using substring complements $\COMPS{n}$.
In fact, $\GrayDecision{\BINARY{n}}{\COMPS{n}}$ is strongly NP-complete.
\end{theorem}
\begin{proof}
Consider the following set of binary strings from $\BINARY{2n-1}$,
\begin{equation} \label{eq:binaryComplement}
    B_n = \{ \bits{b_1} \padding{1} \bits{b_2} \padding{1} \ldots \padding{1} \bits{b_n} \}
\end{equation}
where each $\bits{b_i}$ implements the single bit.
The padding bits $\padding{1}$ ensure that the only substring complements that can modify $B_n$ are single bit complements.
This is because any substring complement of length $\geq 2$ will include at least one of the padding bits, which will be complemented by the operation, and hence the resulting string will be pushed outside of the $B_n$ set.
\end{proof}

Aaron: what else could we consider for binary strings?
Or perhaps we remove this section?


==> unused/bitFlipsHardOld.tex <==
%%% Our original section for proving our first hardness result

\section{Bit Flip Problem is NP-complete}
\label{sec:bitFlip}

In this section we prove our foundational hardness result.
The decision problem $\BinaryFlipI{S}$ asks if a subset of binary strings $S \subseteq \BINARY{n}$ can be sequenced so that each string is transformed into the next by complementing a single bit.
The decision problem is equivalent to determining if an arbitrary induced subgraph of the $n$-cube $\CubeGraph{n}$ has a Hamilton path. 
We'll prove that this problem is strongly NP-complete by a reduction from the grid graph Hamilton path problem.
Our approach is illustrated in Figure \ref{fig:bitFlips}.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering 
        \raisebox{2em}{\includegraphics[scale=0.35]{GridGraph}}
        \caption{Grid graph $G[P]$ with $r = 8$ and $c = 5$.}
        \label{fig:bitFlips_graph}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.38\textwidth}
        \centering 
        \includegraphics[scale=0.35]{GridRowColumn}
        \caption{Row encodings from $0^{r-1}$ to $1^{r-1}$ and column encodings from $0^{c-1}$ to $1^{c-1}$.}
        \label{fig:bitFlips_rowColumn}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.35\textwidth}
        \centering 
        \raisebox{1em}{\includegraphics[scale=0.7]{GridStrings}}
        \caption{Binary strings $S \subseteq \BINARY{11}$ associated with $P$, where $(r-1)+(c-1) = 11$.}
        \label{fig:bitFlips_strings}
    \end{subfigure}
    \caption{Illustrating the reduction from $\HPGrid{P}$ to $\BinaryFlipI{S} = \BinaryI[\BITFLIPS{n}]{S} = \GrayI[\BINARY{n},\BITFLIPS{n}]{S}$.
    For example, the rightmost point in the top row in (a) is at position $(2,7) \in P$ and it corresponds to $\blue{1111111}\red{0011}$ in $S$.
    The Hamilton paths in $G[P]$ and Gray code listings of $S$ are in bijective correspondence.
    Aaron: The reduction is parsimonious!}
    \label{fig:bitFlips}
\end{figure}

\begin{theorem} \label{thm:bitFlips}
The decision problem $\BinaryFlipDP$ is strongly NP-complete.
In other words, it is difficult to determine if an arbitrary induced subgraph of the $n$-cube has a Hamilton path. 
\end{theorem}
\begin{proof}
Consider an arbitrary instance of the source problem, $\HPGrid{P}$, where $P$ is in standard position and has $k$ points.  
Let $c-1$ and $r-1$ be the maximum $x$ and $y$ values in $P$, respectively.  
In other words, $P$ spans $r$ rows and $c$ columns of the infinite grid.

First we check if the grid graph $G[P]$ is connected.
If not, we immediately answer no, since $G[P]$ cannot have a Hamilton path.
This pre-processing step can be done in polynomial-time with respect to the size of the input, so it is ``free'' with respect to our polynomial-time reduction.
A consequence of this step is that we may assume that $k \geq r$ and $k \geq c$, since $G[P]$ is disconnected if there are any empty rows and columns.
This assumption will be helpful when we justify that our reduction runs in polynomial-time.

We construct a subset of binary strings $S \subseteq \BINARY{m}$ with $m = (r-1) + (c-1)$.
The size of the subset is $|S| = k$, with each point in $P$ contributing one string to the subset.
Each string consists of a prefix of length $r-1$ which is based on the point's row, followed by a suffix of length $c-1$ which is based on the point's column.
More specifically, the rows and columns are encoding using strings from $R$ and $C$ below, respectively, 
\begin{align*}
R = \{\blue{0^{r-1}}, \blue{10^{r-2}}, \blue{110^{r-3}}, \ldots, \blue{1^{r-1}}\} && C = \{\red{0^{c-1}}, \red{0^{c-2}1}, \red{0^{c-3}11}, \ldots, \red{1^{c-1}}\}
\end{align*}
where exponentiation denotes concatenation.
Precisely, the set $S$ is defined below.
\begin{equation} \label{eq:peakless}
S = \{ \blue{1^x 0^{r-x-1}} \red{0^y 1^{c-y-1}} |  (x, y) \in P \}
\end{equation}
We say that the string $\blue{1^x 0^{r-x-1}}  \red{0^{c-y-1} 1^y}  \in S$ corresponds to the point $(x, y) \in P$, and vice versa.  
Now we prove that $\HPGrid{P}$ and $\BinaryFlipI{S}$ have the same answer.

Suppose that $\HPGrid{P}$ is yes.  
Therefore, $G[P]$ has a Hamilton path.  
Let $H = (x_1, y_1), (x_2, y_2), \ldots, (x_k, y_k)$ be an order of the points in a Hamilton path.  
Let $C$ be the corresponding order of strings in $S$.  
We claim that $C$ is a Gray code.  
To prove this, we start by noting that in $H$, each consecutive pair of points $(x, y), (x', y')$ differ by one in either the $x$ or $y$ coordinate.  
In the former case, we know that $x' \in \{x-1, x+1\}$ and $y' = y$.  
Therefore, there are only two possibilities for the consecutive pair of corresponding binary strings:
\begin{itemize}
    \item $\blue{1^x 0^{r-x-1}}  \red{0^{c-y-1} 1^y}$ is followed by $\blue{1^{x-1} 0^{r-x}}  \red{0^{c-y-1} 1^y}$.
    \item $\blue{1^x 0^{r-x-1}}  \red{0^{c-y-1} 1^y}$ is followed by $\blue{1^{x+1} 0^{r-x-2}}  \red{0^{c-y-1} 1^y}$.
\end{itemize}
In both cases, this is a valid Gray code change, since only a single bit is modified.  
A similar argument handles the case in which the y coordinate differs.
Therefore, $C$ is a Gray code.

Suppose that $\BinaryI{S}$ is yes.  
Therefore, $S$ has a Gray code $C = b_1, b_2, \ldots, b_k$.  
Let $H$ be the corresponding order of points in $P$.  
We claim that $H$ is an order of points on a Hamilton path in $G[P]$.  
Consider a consecutive pair of strings, $b_{i} = \blue{\alpha} \red{\beta}$ and $b_{i+1} = \blue{\alpha'} \red{\beta'}$, where $|\red{\alpha}| = |\red{\alpha'}| = r-1$ and $|\blue{\beta}| = |\blue{\beta'}| = c-1$.
Only a single bit changes between $b_{i}$ and $b_{i+1}$, so either $\blue{\alpha} = \blue{\alpha'}$ and $\red{\beta} \neq \red{\beta'}$, or $\blue{\alpha} \neq \blue{alpha'}$ and $\red{\beta} = \red{\beta'}$.  
Let us consider the former case.  
In this case, we also know that only a single bit changes between $\red{\beta}$ and $\red{\beta'}$.  Furthermore, based on the suffix set $B$ from \eqref{eq:encodePrefixSuffix}, there are two possibilities for the pair of corresponding points:
\begin{itemize}
    \item $(x, y)$ is followed by $(x', y')$ where $x' = x - 1$ and $y' = y$ (i.e. a move to the left), or
    \item $(x, y)$ is followed by $(x', y')$ where $x' = x + 1$ and $y' = y$ (i.e. a move to the right).
\end{itemize}
In both cases, $(x, y)$ and $(x', y')$ are adjacent in $G[P]$.  
A similar argument handles the case when the prefix changes, with the two possibilities translating to up and down moves in the graph.  
Therefore, $H$ is an order of points around a Hamilton path.

Aaron: add membership in NP.
\end{proof}

Aaron: we need to discuss encoding of $S$ as well 
and note that $|S|$ refers to the number of strings in $S$
wait, does $|S|$ vs encoding size of $S$ matter?
what if there is a constant number of long strings in $S$? 
can we answer the problem in polynomial-time in these cases?
does it matter?

\subsection{Hypercube Reductions}
\label{sec:bitFlip_reductions}

Given our foundational hardness result on $\BinaryFlipDP$, we can prove that other problems are NP-hard by reducing them to it.
More specifically, we will use a strategy that we refer to as a \emph{hypercube reduction}.
This strategy shows that the flip graph of interest contains induced subgraphs that are isomorphic to hypercubes.
As a result, we can reduce $\BinaryFlipDP$ to the decision problem of interest.
The resulting meta-theorem is stated and proven below.

\begin{theorem}[Hypercube Reductions]
\label{thm:hypercubeReduction}
Let $\graph{G} = \flipGraph{\objSet{O}_m}{\flipSet{F}_m}$ be a flip graph.
Suppose that its induced subgraph $\graph{G}[\objSet{X}_m]$ is isomorphic to the $n$-cube $\CubeGraph{n}$ for some $\objSet{X}_m \subseteq \objSet{O}_m$.
Then 
\begin{equation} \label{eq:hypercubeReduction}
\BinaryFlipI{S} = \GrayI[\objSet{O}_m,\flipSet{F}_m]{S'} \text{ for all } S \subseteq \BINARY{n}
\end{equation}
where $S' \subseteq \objSet{X}_m$ are the objects corresponding to $S$.
Moreover, if $S'$ can be computed from $S$ in polynomial-time (relative to the encoding size of $S$) then $\GrayDP{\objSet{O}_m,\flipSet{F}_m}$ is strongly NP-complete.
% Note: $O(p(|S|))$-time for some polynomial function $p$ is not equivalent to what is written above.
% This is because $|S|$ (i.e., the quantity of strings in $S$) isn't always polynomially related to the encoding size of $S$.
% In particular, if $S$ contains a constant number of long strings, then the encoding of $S$ is dominated by the string length and not the quantity.
% Note: In particular, this implies that $m \in O(q(n))$ for some polynomial function $q$
\end{theorem}
\begin{proof}
Consider $\BinaryFlipI{S}$ for some $S \subseteq \BINARY{n}$, and let $S' \subseteq \objSet{X}_m \subseteq \objSet{O}_m$ be the objects corresponding to $S$.
Since $\graph{G}[\objSet{X}_m]$ is isomorphic to the $n$-cube $\CubeGraph{n}$, this means that $\graph{G}[S']$ is isomorphic to $\CubeGraph{n}[S]$.
Therefore, $\CubeGraph{n}[S]$ is Hamiltonian if and only if $\graph{G}[S']$ is Hamiltonian.
Hence, \eqref{eq:hypercubeReduction} holds.
Moreover, if $S'$ can be computed from $S$ in polynomial-time (relative to the encoding size of $S$), then we can map $\BinaryFlipI{S}$ to $\GrayI[\objSet{O}_m,\flipSet{F}_m]{S'}$ in polynomial-time.
Thus, strong NP-completeness follows from Lemma \ref{lem:NP}.
\end{proof}

Hypercube reductions can be described in one of two ways:
\begin{itemize}
    \item \emph{Scaling down} starts with a flip graph and identifies an induced subgraph that is isomorphic to $\CubeGraph{n}$.
    \item \emph{Scaling up} starts with an $n$-cube $\CubeGraph{n}$ and modifies its labels to be an induced subgraph of another flip graph.
\end{itemize}
Only one of these approaches is necessary when applying Theorem \ref{thm:hypercubeReduction}.
However, in some cases we will provide both viewpoints, and take for granted that their equivalence is self-evident.
All of our mappings are very simple, so we omit justification that 
% also \emph{implementing} a bit and \emph{constraining the operations}


==> unused/finalOld.tex <==

In this paper, we set out to investigate whether or not Gray code results can be fortified by any underlying issues of complexity.

The authors were initially surprised by how many problems were so easily amendable to this approach.
In other words, we didn't expect to be able to find induced hypercubes in so many other well-structured graphs.
In retrospect, this is less surprising, as 

The approach often works when the objects and operations support independent local modifications, or more specifically, \emph{independent involutions}.
By this we mean that changes can done and undone (i.e., there are self-inverse or \emph{involution} operations) and they are \emph{independent} in the sense that they don't affect other potential changes.
There is some irony in independent involutions leading to hardness, as they have been at the core of Gray code creation since the binary reflected Gray code.

Moving forward, the authors hope that this work will be incorporated into future investigations of Gray codes as follows.
\begin{itemize}
    \item Authors will consider the complexity of the underlying problem and refer to it as the \emph{subset Gray code problem}, or simply the \emph{subset problem}.
    \item If the objects and operations support independent involutions, then authors will attempt to perform a hypercube reduction to establish hardness of the subset problem.
\end{itemize}
With regard to the second point, we suggest that authors can simply specify the family of subset of objects that induce hypercubes of any order $n$.
Those wishing to ``double-check'' their reduction are welcome to contact the authors of this paper.

\subsection{Additional Results}
\label{sec:final_additional}

It is worth noting that some important subset problems can be proven to be solvable in polynomial-time.
Aaron: move de Bruijn sequence material here?

Many additional results have been left on the table, so to speak.
For example, the set of strings considered in \eqref{eq:rotationSet} will also work for \emph{unlabelled necklaces} (and variants) where the underlying equivalence allows for symbol remapping (i.e., complementation in the binary case).
Similarly, some of our approaches can be combined to create further results.
For example, the ideas presented for combinations in Section \ref{sec:combos} and rotational objects in Section \ref{sec:rotation} can be combined to create hardness results for fixed-weight necklaces (and variants).
In future work we will also strengthen many of our stated results by considering future restrictions on the operations (e.g., substring reversals or rotations of length $\geq k$). 

Careful readers will have noticed that our reductions are all \emph{parsimonious} in the sense that they preserve the number of solutions (and not just whether there is a solution or not).
For this reason, our results have implications for ASP-hardness \cite{yato2003complexity}.

For simplicity, we focused our attention on Hamilton paths and the resulting hardness of (linear) subset Gray code problems.
Similar results can be derived for \emph{cyclic Gray codes} (i.e., where the last object can be transformed into the first object using one of the allowed operations) using Hamilton cycles.
% We also did not consider the hardness of $k$-Gray codes where consecutive objects differ by at most $k$ operations.
% Finally, 
There may also be interest in Gray code problems that specify the starting and and ending object, and our general approach can be adapted to establish hardness for these problems.

\subsection{Future Work}
\label{sec:final_future}

The authors considered several types of subset problems for which hypercube reductions didn't seem possible.
In these cases, one could prevent futile consideration by formally proving that the underlying flip graph does not contain hypercubes of sufficient size as induced subgraphs.
To complement this direction, it would be helpful to develop similar reductions using a graph other than the hypercube.

The authors plan to build on this work by investigating optimization and approximation problems.
For example, the following questions are natural for a subset of $n$-bit binary strings.
\begin{itemize}
    \item What is the longest Gray code that can be constructed using a subset of the provided strings?
    \item What is complexity of finding a Gray code that uses a given fraction of the provided strings?
\end{itemize}


\subsection{Open Problems}
\label{sec:final_open}

As mentioned above, we were unable to establish the hardness for certain subset problems.
In this space, we highlight two specific challenges.
Fittingly, they involve two of the most stubborn Gray code problems that were solved during the past decade:
the middle levels \cite{mutze2016proof} and sigma-tau problems \cite{sawada2019solving}.

\subsubsection{Global Constraints}
\label{sec:final_open_global}

The \emph{middle-levels conjecture} asserted the existence of a Hamilton cycle in middle two levels of the hypercube of order $n=2k+1$.
In other words, there is a bit-flip Gray code of $\COMBOS{n}{k} \cup \COMBOS{n}{k+1}$.
In this context, it is clear that the operations are involutions.
However, they do not meet the independent involution criteria discussed at the start of Section \ref{sec:final}.
This is because the operations must alternate between flipping $0$ to $1$ and flipping $1$ to $0$.
In other words, flipping a $0$ to $1$ will prevent any flips in the same direction from being performed next.

Another way of viewing this issue is that there \emph{global constraints} placed on the operations.
More specifically, one can only flip $0$ to $1$ in objects from $\COMBOS{n}{k}$, and flip $1$ to $0$ in objects from $\COMBOS{n}{k+1}$.
Hypercube reductions don't seem to be applicable in situations such as these.

\subsubsection{Prefix Operations}
\label{sec:final_open_prefix}

The \emph{sigma-tau problem} asked if the permutations of $[n]$ can be ordered by swapping the first two symbols (i.e., $\tau = (1 \ 2)$) or rotating the entire permutation one position to the left (i.e., $\sigma = (1 \ 2 \ \ldots \ n)$).
While $\tau$ is an involution, it is the only allowable involution.
These two operations are examples of \emph{prefix operation} as they modify the symbols in some prefix of the underlying object.
In particular, they always modify the first symbol.
As a result, they don't support the notion of independent involutions since (a) there is only one involution, and (b) the operations are not independent since they always overlap each other.

In this case, one must consider the possibility that the underlying subset problem can be solved in polynomial-time.
To support this possibility, note that when the operations are $\sigma$ and $\sigma' = (1 \ 2 \ \ldots \ n{-}1)$ the subset problem is equivalent to finding a shorthand universal cycle (e.g., see \cite{holroyd2012shorthand}) and this can be decided in polynomial-time.

% for example, careful readers note that not shift operations.
% for example, we provided underlying hardness results for \cite{wang1996gray} and \cite{ueda2000gray}, but not \cite{sawada2013gray}.
% sigma tau.
% there is an involution.
% other operations are not independent.
% more broadly, prefix shifts.
% and prefix operations.
% irony here is that seemingly difficult Gray code problems we have not proven hard here.

% Aaron: our meta-theorem does not seem to work for prefix operations 
% e.g., prefix-reversals; see \cite{essed2014harassed,sawada2016greedy,cameron2022hamiltonicity}.
% e.g., prefix-rotations; see \cite{williams2009loopless,williams2009shift}.
% e.g., star transpositions; see \cite{}

% must confront the possibility that these problems can be solved in polynomial-time.
% subsets of prefix-rotations seem particularly prone to polynomial-time solvability.
% this includes  n-1 and n mentioned in Section \ref{sec:back_deBruijn} 
% is sigma-tau poly-time; see \cite{sawada2018hamilton,sawada2019solving} which has a simple structure \cite{rytter2021syntactic}?
% What about other subsets of prefix-rotations, 
% e.g. yes for 2,3,n for permutations; see \cite{stevens2012hamilton}
% e.g. no for combinations 2, n, -n; see \cite{cheng2007generating}




==> unused/introOld.tex <==
%%% This contains an earlier version of our intro
%%% It includes several things that we want to save
%%% including related work and a table summarizing our results

\section{Introduction OLD}
\label{sec:oldIntro}

In modern times, the clever ordering of binary strings dates back to the work of Émile Baudot and Frank Gray.  
Both engineers devised a way to order the $2^n$ binary strings of length $n$ so that consecutive strings differ in only one bit.  
Their order became known as the \emph{(binary reflected) Gray code}, in part due to a patent filed by Gray.  
The same order is also implicit in much earlier puzzles including the Chinese Ring puzzle (also known as Baguenaudier or ``time-waster''), and later puzzles like the Towers of Hanoi and Spin-Out.

While the binary reflected Gray code is a cute (and useful) bit of combinatorial and computational mathematics, similar pursuits can be incredibly challenging.  
For example, the well-known middle levels conjecture asked if the same type of ordering exists for the binary strings of length $2k+1$ that have either $k$ or $k+1$ copies of $1$.  
This conjecture had been given a difficulty rating of 49/50 by Knuth, and was settled in the affirmative by Mütze.  
More recently, this result was generalized to central levels by Gregor, Mička, and Mütze.
When viewed as a graph, these problems are based on the existence of Hamilton paths in induced subgraphs of the n-cube.  
Specifically, the Gray code is a Hamilton path in the full $n$-cube, while the middle levels solution is a Hamilton path in the $(2k+1)$-cube induced on vertices with weight $k$ or $k+1$; the central levels solution generalizes these two results by considering vertices with weight $k-c, k-c+1, \ldots, k+c, k+c+1$ for any $1 \leq c \leq k$.

Few variants of similar problems are still open. 
A necklace is an equivalence
class of binary strings under rotation. For a~$n$ bit binary string~$x_1\cdots x_n$, we define the rotation operation~$\sigma(x_1x_2\cdots x_n) = x_2\cdots x_nx_1$. We say that bitstrings $x$ and $y$ are in the same necklace if and only if~$\sigma^i(x) = y$ for some integer
$i$. A necklace is identified by specifying any one of its elements and frequently the
lexicographically smallest string is chosen as the representative. 
For even values of~$n$, a 1-Gray code (where the consecutive bitstrings differ at one position or a single bit flip) for necklaces does not exist due to balancedness problems
(regardless of the choice of representatives); see~\cite{MR1413286}. However, for odd values of~$n$ this problem is still open.

In this paper, we show that the natural decision problem underlying these results is NP-complete.  
In other words, in general it is NP-complete to decide if a given induced subgraph of the $n$-cube has a Hamilton path (or cycle).  
When translated to the binary strings, our result implies the following: 
It is NP-complete to decide if a set of $n$-bit binary strings has a Gray code order where two consecutive entries differ by a single bit flip. 
In fact, in a much stronger result, we will show that this holds even when the set is restricted to ~\emph{peakless binary strings} of the form~$1^* 0^* 1^*$.

We prove the NP-hardness of deciding if a given induced subgraph of the n-cube has a Hamiltonian path (or cycle)
by reducing it from the Hamiltonicity problem on a grid graph with holes. For the positive integers~$m$ and~$n$, the vertex set~$V$ and the edge set~$E$, rectangular grid graph~$G(m, n)$ is defined as follows:
~$V = \{(i, j) \mid 1 \leq i \leq m, 1 \leq j \leq n\}$ and
~$E = \{(u, v) \mid u, v \in V \text{and} \, |u_i - v_i| + |u_j - v_j| = 1\}$. It was proved in~\cite{itai1982hamilton} that it is NP-complete to decide whether the graph~$G(m, n)$ has a Hamiltonian path (or cycle). 

Let~$\BINARY{n}$ be the set of all binary strings of length~$n$. For any~$S \subseteq \BINARY{n}$, the decision problem~$\BinaryFlipDP(S)$ asks if all binary strings in~$S$ can be ordered such that consecutive strings differ by a bit flip. In our first result, we prove that~$\BinaryFlipDP$ is NP-complete.
\begin{theorem}
The decision problem $\BinaryFlipDP$ is strongly NP-complete.
In other words, it is NP-complete to determine if an arbitrary induced subgraph of the $n$-hypercube has a Hamilton path.
\label{thm:binary-hardness}
\end{theorem}

Our first Theorem~\ref{thm:binary-hardness} is then used as a basis to show NP-completeness of variety of other problems. In such problems instead of binary strings, we have other combinatorial objects like permutations, combinations, spanning trees, matchings, necklaces, binary trees, etc. Moreover, we use variety of operations on such objects. In the next result, we prove NP-completeness of a problem that asks for a given set of objects, is there a way to order them such that two consecutive objects differ by some specified operation.
\begin{theorem}
It is NP-complete to determine if an arbitrary set of objects can be ordered such that two consecutive objects differ by some specified operations.
We summarize the objects and their respective operations in Table~\ref{tab:ob-and-oper}. 
\begin{table}
    \centering
    \begin{tabular}{c|c}
        Objects & Operations \\ \hline
        Binary strings & bit flips, substring complements\\
        Combinations & swaps, substring reversals, substring rotations \\
        Permutations & swaps, substring reversals, substring rotations, jumps \\
        Spanning trees & edge exchanges \\
        Binary trees & edge rotations
    \end{tabular}
    \caption{Objects and their respective operations.}
    \label{tab:ob-and-oper}
\end{table}
\label{thm:ob-and-oper}
\end{theorem}

We prove the results in Theorem \ref{thm:ob-and-oper} using \emph{hypercube reductions}.
Informally, these reductions involve finding hypercubes as induced subgraphs.
For example, consider the problem of ordering the non-crossing partitions of $[n] = \{1,2,\ldots,n\}$ by either dividing one part of the partition into two, or combining two parts into one.
This Gray code problem is equivalent to finding a Hamilton path in the \emph{refinement poset} shown in Figure \ref{fig:noncrossing_hasse4}.
This graph contains a hypercube of order $3$ as an induced subgraph, as shown in Figure \ref{fig:noncrossing_subgraph}--\ref{fig:noncrossing_cube3}.
More generally, Section \ref{sec:cat} shows that the hypercube of order $n$ can always be found as an induced subgraph of the refinement poset of order $n+1$.
Therefore, an induced subgraph of the hypercube of degree $n$ is isomorphic to an induced subgraph of the refinement poset of order $n+1$.
Hence, Theorem \ref{thm:binary-hardness} implies Theorem \ref{thm:ob-and-oper} for non-crossing partitions using these operations.
% A partition α of a set X is a refinement of a partition ρ of X—and we say that α is finer than ρ and that ρ is coarser than α—if every element of α is a subset of some element of ρ. Informally, this means that α is a further fragmentation of ρ. In that case, it is written that α ≤ ρ.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.42\textwidth}
        \includegraphics[scale=1.2]{noncrossingPoset4}
        \caption{The Hasse diagram of non-crossing partitions of $[n+1]=[4]$ under refinement.}
        \label{fig:noncrossing_hasse4}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.34\textwidth}
        \includegraphics[scale=1.2]{noncrossingPoset4Subgraph}
        \caption{An induced subgraph of the Hasse diagram from (a).}
        \label{fig:noncrossing_subgraph}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.21\textwidth}
        \includegraphics[scale=1.2]{noncrossingPoset4Cube3}
        \caption{(b) is isomorphic to the cube of order $n=3$}
        \label{fig:noncrossing_cube3}
    \end{subfigure}
    \caption{
    Illustrating a hypercube reduction.
    }
    \label{fig:noncrossing}
\end{figure}


The authors were motivated by the following observation. 
There are numerous papers in the literature that prove the existence or non-existence of a Hamilton paths in a specific graph or
alternatively, Gray code results on particular sets of combinatorial objects using an allowable set of operations. These results and related open problems are systematically compiled in an excellent survey on combinatorial Gray codes by M\"utze; see~\cite{mutze2022combinatorial}.

%Although these individual problems can be extremely challenging, they are often uninteresting from the vantage point of computational complexity.  
In some cases the answer to these problems tends to be uniformly yes or no.  
In other cases, the answer is quite out of reach.
An example of the later case includes the Lovász's conjecture from 1970s that states that all vertex-transitive graphs have a Hamilton cycle, except for the five graphs. Recently, some interesting families of vertex-transitive graphs were shown to contain a Hamilton cycle. Specifically, the Kneser graphs, denoted by~$K(n,k)$ has as vertices all~$k$-element subsets of an~$n$-element ground set, and an edge between any two disjoint sets, were proved by Hamiltonian; see~\cite{merino2022kneser}. This was also an open problem since 1970s.
Another such result is the recent solution to sigma-tau problem, which asked if permutations can be ordered so that consecutive permutations differ by a swap of the first two elements or a left-rotation of the entire permutation; 
Sawada and Williams proved that there is a linear order when~$n$ is even and a cyclic order when~$n$ is odd; see~\cite{sawada2018hamilton}.

The focus of this paper is to study these purely combinatorial problems from the lens of computational complexity. We want to understand how hard or easy it is to generate a given set of objects such that two consecutive objects differs by some measurable amount. For example, a decision version of Hamiltonicity problem in Kneser graphs can be stated as: given a set of all~$k$-element subsets of an~$n$-element ground set. Can we order the sets such that any two consecutive sets are disjoint. In the paper, we study many such decision problems and produce a standard framework to prove hardness results for different combinatorial generation problems. In the standard framework, we reduce a given set of objects and the specified operation to an induced subgraph in a hypercube.

\subsection{Related Work}
\label{sec:oldIntro_related}

The complexity of enumeration in general has been studied widely and there already exists a rich collection of complexity classes in the enumeration complexity zoo. In the analysis of enumeration algorithms, we
evaluate the total time to compute all solutions with respect to the size of both the input and the output. Algorithms whose complexity is given in this fashion are often called output-sensitive. Fundamental complexity notions for enumeration have been proposed 30
years ago by Johnson, Yannakakis and Papadimitriou~\cite{MR933271}. In recent years, the enumeration complexity has been studied in more details. We point to the survey~\cite{CS19}, where time and space complexity classes for enumeration problems have been studied. Some of the notable time classes include polynomial delay DelayP, incremental polynomial time IncP and output polynomial time OutputP. 
The classes~DelayP$^{poly}$ and~IncP$^{poly}$ are
the class of problems solvable in polynomial delay and polynomial space and the class of problems solvable in incremental polynomial time and polynomial space, respectively. 
The complexity landscape for enumeration problems in DelayP has been   refined further by introducing very low classes defined
by using Boolean circuits as enumerators~\cite{creignou2022enumeration}.

In this paper, we prove that deciding whether an induced subgraph of a hypercube is Hamiltonian is NP-complete. The following complementary problem is also known to be NP-hard: given a set of binary strings~$S' \subseteq \BINARY{n}$, does the subgraph induced by~$\BINARY{n} \setminus S'$ has a Hamiltonian cycle?
Apart from this question, various different variants related to the hypercube subgraphs were considered in~\cite{dvovrak2012gray}.

We prove Theorem~\ref{thm:binary-hardness} by reducing~$\BinaryFlipDP$ from the Hamiltonicity problem in a grid graph with holes. These grid graphs and their variants constitute quite a popular class of graphs to study Hamiltonicity and there has been a tremendous amount of work in this direction; see the survey by Arkin and others~\cite{arkin2009not}.
Aaron: poly-time solvable for solid grid graphs~\cite{umans1997hamiltonian}

The proof of Theorem~\ref{thm:ob-and-oper} follows by finding an arbitrary induced hypercubes within the larger hypercubes, permutohedra, and flip graphs defined by other combinatorial objects and the specified operations. In a flip graph, vertices are the combinatorial objects and there is an edge between two objects if they differ by a specified operation.
In general, looking for a subgraph in another graph is a rich area of research. Arguably one of the most important theorems in graph theory namely, Robertson-Seymour states that every family of graphs that is closed under minors can be defined by a finite set of forbidden minors; see \cite{robertson2004graph}. They published a series of twenty papers spanning over 500 pages from 1983 to 2004.

Various researchers also studied graph colouring, which is another fundamental concept
of graph theory in family of graphs defined by subgraphs in a certain way.
A graph family~$P$ is hereditary or induced-hereditary if, for any graph~$G \in P$, all its subgraphs or induced-subgraphs, respectively, are also in ~$P$. A
property is additive if for any two graphs~$G, H \in P$,
their disjoint union is also in~$P$.  Let~$P_1, \ldots ,P_k$ be graph families with~$k > 1$. A graph~$G = (V, E)$
is~$(P_1, \ldots , P_k)$-colorable if there is a partition~$(V_1, \ldots , V_k)$ of~$V(G)$ such that~$G[V_i] \in P_j$ for each~$i = 1, \ldots , k.$ The problem of recognizing~$(P_1, \ldots , P_k)$-
colorable graphs is usually referred to as Generalized Graph Coloring; see~\cite{brown1996complexity}.  
Alekseev, Farrugia and Lozin proved that if
all~$P_i$s are additive induced-hereditary, then the generalized graph coloring is
NP-hard, with the only exception of bipartite graphs; see~\cite{farrugia2003uniqueness} and~\cite{lozin2004new}.

% Vertex-partitioning into fixed additive induced-hereditary properties is NP-hard
Another classical problem in theoretical computer science, the subgraph isomorphism problem is a computational task in which two graphs~$G$ and~$H$ are given as input, and we determine whether~$G$ contains a subgraph that is isomorphic to~$H$; see~\cite{ullmann1976algorithm}.


Ask Aaron!!
mention cottage industries,
Also see Eduardo's paper, ASP-hardness, parsimonious reductions, counting complexity, number of Hamilton paths.
%On the theorem of Fredricksen and Maiorana about de Bruijn sequences



\subsection{Overview}
When discussing a particular Gray code problem, we'll cite previous results that deal with the full set of objects, including Gray codes and enumerative results.
For example, when discussing bit flips, the binary reflected Gray code \cite{gray1953pulse} and de Bruijn sequences \cite{de1946combinatorial}...

Do this for specific sections you are writing.

Sections etc.


==> unused/operationLengthOld.tex <==
%%% Discussion of operation length in an older style

\subsection{Substring Rotations of length atleast 3}
In this case, we reduce the problem from~$k-$ary Gray code. Let~$\mathcal{G}_n$ be the set of general~$k$-ary Gray code. Thus, for~$X \in \mathcal{G}_n$ and for any~$i$,~$X_i$
has~$k$ many choices. We  reduce it from the problem~$\GrayProblem{\mathcal{G}_n}{O}$. We consider a substring of length~$k$ and corresponding to each~$X_i$, we associate an unique rotation of the substring of size~$k$. Since there are~$k$ unique rotations for  substring of length~$k$, we can associate each choice of~$X_i$ with one of the rotated substring. We take anti-clockwise rotations without a loss of generality.
Thus, if  two consecutive strings of a~$k$-ary Gray code differs by +1/-1, the corresponding permutations differs by a substring rotation of length~$k$.
Example with ternary code:

        000    123456789 \\
        010    123645789 \\
        020     123564789  \\  

In this case, all  two consecutive permutations differs exactly by substring rotation of length 3.
So, if atleast k is asked we encode a single element of the string by k length substring in a permutation.


\subsection{Jumps of length atleast 3}
The idea is still to use K-ary code though. The mapping will be different. We will start with a substring of length~$k$ and identity permutation 1234$\cdots k$. So corresponding to~$k$ choices of~$X_i$, we have~$k$ substring such that the highest element~$k$ is at all possible~$k$ positions in substring 

Consider the following example : 

0     1234

1     1243

2     1423

3     4123



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.275\textwidth}
        \centering 
        \raisebox{5em}{\includegraphics{binarySubstringComplement}}
        \caption{Mapping $\purple{10100} \in S$ to $\purple{1}1\purple{0}1\purple{1}1\purple{0}1\purple{0} \in S'$.}
        \label{fig:appendixBitSubs_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.575\textwidth}
        \centering 
        \includegraphics{binarySubstringComplement3}
        \caption{If we don't allow substring complements of length $\leq 2$, then we map $\purple{10100} \in S$ to $\purple{111}1\purple{000}1\purple{111}1\purple{000}1\purple{000} \in S'$.}
        \label{fig:appendixBitSubs_3}
    \end{subfigure}
    % \begin{subfigure}[b]{0.575\textwidth}
    %     \centering 
    %     \includegraphics{binarySubstringComplement3}
    %     \caption{If we don't allow substring complements of length $\leq 2$, then we map $\purple{10100} \in S$ to $\purple{111}1\purple{000}1\purple{111}1\purple{000}1\purple{000} \in S'$.}
    %     \label{fig:bitComp_3}
    % \end{subfigure}
    \caption{Reducing a bit complement problem $\GrayI[\BINARY{n},\BITFLIPS{n}]{S}$ to a substring complement problem $\GrayI[\BINARY{n},\COMPS{n}]{S'}$.}
    \label{fig:appendixBitSubs}
\end{figure}


==> unused/outtakes.tex <==

%%% Older version of abstract

\begin{abstract}
    
It is well-known that the $n$-cube has a Hamilton path.
In particular, the venerable binary reflected Gray code provides one such cycle.  
Recently, it was proven that the middle two levels of the (2k+1)-cube has a Hamilton path.  
In that case, the result settled a famous open problem that had been assigned a difficulty of 49/50 by Knuth.  
In this paper, we view the underlying existence questions as special cases of the following decision problem: 
Does a given induced subgraph of the n-cube have a Hamilton path?  We prove that this decision problem is NP-Complete.  
When translated to the vertex labels, our result implies the following: It is NP-Complete to decide if a set of n-bit binary strings has a Gray code.  
In fact, we prove a much stronger result: The aforementioned Gray code decision problem is NP-Complete even when the set of strings is restricted to the peakless strings of the form $1^* 0^* 1^*$.

Our approach also lends itself quite easily to a number of similar decision problems.  
For example, it is NP-Complete to decide if there is a Hamilton path in a given induced subgraph of the permutohedron.  
In this case, the corollary is the NP-Completeness of deciding if a set of permutations has an adjacent-transposition Gray code.  
When the input to these decision problems is a set of strings (as opposed to a graph), we obtain strong NP-Completeness, and not weak NP-Completeness.  
Our results also apply to Hamilton cycles. 

% But how difficult are they in terms of computational complexity?
% provides some theoretical basis for countless papers in the literature
\end{abstract}


%%% Old substring complement subsection with figures

We'll prove that $\CompGraph{m}[S]$ suffices for $m=2n-1$ and the following subset,
\begin{equation} \label{eq:compMap}
S = \{b_1 b_2 \ldots b_{2n-1} \mid b_i = 1 \text{ if $i$ is even.}\}
\end{equation}
In other words, we simply induce the substring complement graph of odd-order on the vertices that have $\pad$ in every second position.
This is illustrated in Figure \ref{fig:binaryComplement} and proven in Lemma \ref{lem:bitComp}.


\begin{figure}[h]
    \centering 
    \begin{subfigure}[t]{0.725\textwidth}
        \centering 
        \includegraphics{compScaleDown3}
        \caption{Substring complement graph $\CompGraph{3}$ (left).
        Its induced subgraph $\CompGraph{3}[S]$ using \eqref{eq:compMap} is isomorphic to the hypercube $\CubeGraph{2}$ (right).
        The black, purple, and gold edges correspond to substring complements of length $1$--$3$, respectively.
        }
        \label{fig:binaryComplement_graph3}
        \label{fig:binaryComplement_subgraph5}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \centering 
        \raisebox{2.85em}{\includegraphics{binaryComplementHypercube3}}
        \caption{The induced subgraph $\CompGraph{5}[S]$ isomorphic to $\CubeGraph{3}$.}
        % \caption{Hypercube $\CubeGraph{3}$ as an induced subgraph of $\CompGraph{5}$.}
        \label{fig:binaryComplement_subgraph5}
    \end{subfigure}
    \caption{
    The binary substring complement graph $\CompGraph{m}$ scales down to the $n$-cube $\CubeGraph{n}$ for $m=2n-1$.
    Simply induce on $\CompGraph{m}$'s vertices whose labels have $\pad$ at every even index, as per \eqref{eq:compMap}.
    }
    \label{fig:binaryComplement}
\end{figure}

The previous paragraph describes how to ``scale down'' $\CompGraph{m}$.
Equivalently, we can describe how to ``scale up'' $\CubeGraph{n}$.
We do this by inserting \emph{static bits} as \emph{padding} between each pair of bits.
This is illustrated in Figure \ref{fig:bitComp}.

\begin{figure}[h]
    \begin{subfigure}[t]{0.41\textwidth}
        \centering 
        \includegraphics{compMapString}
        \caption{Mapping $\BINARY{n}$ to $\BINARY{m}$ with $m=2n-1$ by interleaving static bits as padding.}
        \label{fig:bitComp_mapString}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.57\textwidth}
        \centering 
        \includegraphics{compMapGraph}
        \caption{Mapping hypercube $\CubeGraph{2}$ with vertex set $\{00,01,10,11\}$ to the induced subgraph $\CompGraph{3}[S]$ with $S = \{0\pad0,0\pad1,1\pad0,1\pad1\}$.}
        \label{fig:bitComp_mapGraph}
    \end{subfigure}
    \caption{
    The $n$-cube $\CubeGraph{n}$ scales up to an induced subgraph of the binary substring complement graph $\CompGraph{m}$.
    Simply add static bits of padding between the bits in $\CubeGraph{n}$'s vertex labels.
    % For example, (a) $10100$ in $\CubeGraph{5}$ maps to $1\pad0\pad1\pad0\pad0$ in $\CompGraph{9}[S]$.
    % The full mapping of $\CubeGraph{2}$ to $\CompGraph{3}[S]$ is in (b).
    }
    \label{fig:bitComp}
\end{figure}

Regardless of how we describe $\CompGraph{m}[S]$, the set $S$ is always anti-closed%
\footnote{An operation is \emph{anti-closed} on a set if applying the operation to any element of the set results in something that is outside of the set.
For example, adding $1$ is anti-closed for the set of even integers.}
under substring complements of length longer than one.
This leads to the following lemma.

\begin{lemma} \label{lem:bitComp}
The hypercube $\CubeGraph{n}$ is an induced subgraph of the binary substring complement graph $\CompGraph{m}$ for $m=2n-1$.
\end{lemma}
\begin{proof}
todo: clean-up this writing ...
more specifically prove for $m=2n-1$ and $S$ from \eqref{eq:compMap} ...
this puts static bit in every even position ...
As a result, the set $S$ is always anti-closed on substring complements of length $>1$ due to the static $\pad$ bits.
this is because any such operation must change a static bit, which pushes the result out of $S$ ...
use Theorem \ref{thm:hypercubeReduction} ...
On the other hand, all substring complements of length $1$ are still valid ...
Thus, the edges in $\CompGraph{m}[S]$ correspond precisely to bit flips...
moreover, all $2^n$ vertices present ...
\end{proof}

Lemma \ref{lem:bitComp} immediately leads to the following corollary.

\begin{corollary} \label{cor:bitComp}
The decision problem $\BinaryCompDP$ is strongly NP-complete.
\end{corollary}

In subsequent sections we employ the hypercube reduction strategy, but with different objects and operations.
In some cases it is easier to describe the ``scale down'' process, while in other cases ``scaling up'' is simpler.
Before completing this subsection, we offer a second proof of Corollary \ref{cor:bitComp} using a standard reduction without the use of the hypercube reduction strategy and Theorem \ref{thm:hypercubeReduction}.

\begin{proof}
We can map $\BinaryFlipI{S}$ to $\BinaryCompI{S'}$ by taking each string in $S$ and interleaving its bits with $1$s to create a corresponding string in $S'$.
This \emph{padding} of static bits ensures that the only valid substring complement changes in $S'$ will be individual bit flips.
Moreover, if the strings in $S$ have length $n$, then the strings in $S'$ will have length $m = 2n-1$.
see Figure \ref{fig:bitComp}...

in other words, we implement each bit using a single bit and then insert $1$s between the bits.
That is, each binary string $b_1 b_2 b_3 \ldots b_{n-1} b_n$ would be mapped to $b_1 \pad b_2 \pad b_3 \pad \ldots \pad b_{n-1} \pad b_n$.
Note that the only valid substring complements are now individual bit complements.
\end{proof}



%%% Substring complements using neighborhood approach
%%% We'll use hypercube approach everywhere instead

\subsection{Substring Complements}
\label{sec:binary_subs}

Let $\bitSub{i}{j}$ the the operation of flipping every bit in the substring of bits $i$ through $j$ for $i \leq j$.
Let $\BITCOMPS{n}$ be the set of all such operations.
The next decision problem that we consider is $\BinaryCompDP = \BinaryDP{\BITCOMPS{n}}$.

Note that this \emph{substring complement} operations include the individual bit flips from Section \ref{sec:binary_flips} as $\bitSub{i}{i} = \bitFlip{i}$.
Thus, if we want to prove that $\BinaryCompDP$ is hard, then it must be that the greater operational flexibility doesn't make the problem tractable.
(If we were to further generalize the operation set to allow any set of bits to be complemented, then the problem would be easy, since any string could be followed by any other string.)

We prove that $\BinaryCompDP$ is hard by reducing $\BinaryFlipDP$ to it.
To map $\BinaryFlipI{S}$ to $\BinaryCompI{S'}$, we take each string in $S$ and interleave its bits with $1$s to create a corresponding string in $S'$.
This \emph{padding} ensures that the only valid substring complement changes in $S'$ will be individual bit flips.
This is illustrated in Figure \ref{fig:bitComp}.


Our proof of correctness will consider the ``neighborhood'' of each string.
With respect to a $\GrayI[\mathcal{O},\mathcal{F}]{S}$ problem, we define the \emph{neighbors} of $s \in S$ as \begin{equation} \label{eq:neighborhood}
    \neighbors[S,\mathcal{F}]{s}
    = \{t \in S | t = f(s) \text{ for some } f \in \mathcal{F}\}.
\end{equation}
A \emph{neighborhood argument} shows that two sets have the same neighborhoods relative to their respective objects and operations.
That is, if there is a bijection $b : S \rightarrow S'$ with $S \subseteq \mathcal{O}$ and $S' \subseteq \mathcal{O'}$, then a neighborhood argument proves that for all $s \in S$
\begin{equation}
\neighbors[\mathcal{O},\mathcal{F}]{s} = \{b^{-1}(t) | t \in \neighbors[\mathcal{O'},\mathcal{F'}]{b(s)}\}
\end{equation}
In other words, the neighbors of $s$ are the same as the neighbors of $b(s)$, relative to the different types of flips.
A neighborhood argument is equivalent to proving that the flip graphs $\flipGraph{\mathcal{F}}{S}$ and $\flipGraph{\mathcal{F'}}{S'}$ are isomorphic according to the vertex bijection $b$.
%(or the induced subgraph of $\flipGraph{\mathcal{F}}{\mathcal{O}}[S]$).
Regardless of how it is viewed, a neighborhood argument is stronger than necessary to prove that the reduction is correct, but it is often an easier result to prove.

\begin{theorem} \label{thm:bitComp}
The decision problem $\BinaryDP{\BITCOMPS{n}}$ is strongly NP-complete.
In other words, it is difficult to determine if an arbitrary set of binary strings has a Gray code order using substring complements.
\end{theorem}
\begin{proof}
Sketch.
Reduce from Bit Flips as follows:
Implement each bit using a single bit and then insert $1$s between the bits.
That is, each binary string $b_1 b_2 b_3 \ldots b_{n-1} b_n$ would be mapped to $b_1 1 b_2 1 b_3 1 \ldots 1 b_{n-1} 1 b_n$.
Note that the only valid substring complements are now individual bit complements.

Aaron: use a neighborhood argument...
\end{proof}



%%% Adfix (i.e. prefix or suffix}
%%% This doesn't work

\subsection{Adfix-Complements}

Aaron: I don't think that there is a way to do this, ooops.

An \emph{adfix} is a prefix or a suffix.
For example, the adfixes of $abc$ are $\{a,ab,abc,bc,c\}$.
% See https://en.wikipedia.org/wiki/Affix
So an \emph{adfix-complement} involves complementing a prefix or a suffix.

Reduction form Grid Graph Hamiltonicity?
i.e., might need gridwise instead of bitwise approach.

Questions:
\begin{itemize}
    \item Can we do this using a reduction from Bit Flips?
    \item We'd like to be able to establish hardness for prefix-complements, but we don't know how handle prefix-based problems.
\end{itemize}


%%% Older section on combinations

\section{Problems on Combinations (OLD)}
\label{sec:combinations}

Combinations are fixed-weight binary strings.
e.g., $\{0111,1011,1101,1110\}$ is a set of combinations.


\subsection{Transpositions and Swaps}

Reduce from Bit Flips as follows:
Implement each bit using two adjacent bits with $01$ for $0$ and $10$ for $1$.
For example, the binary string $0011$ would be mapped to $01 \; 01 \; 10 \; 10$.
Note that the only valid transpositions are local to these pairs of bits.

Also note that this establishes hardness for adjacent-transpositions, which we also refer to as swaps.

Questions:
\begin{itemize}
    \item What about adfix-transpositions (i.e., the first or last symbol is involved in the transposition)?
\end{itemize}

\subsection{Substring Reversals}

Reduce from Bit Flips as follows:
Implement each bit using two adjacent bits with $01$ for $0$ and $10$ for $1$, and then insert some non-palindromic substring between them.
The non-palindromic string can be as short as two bits (e.g., $01$ or $10$) but this makes it harder to differentiate them from the bit-encodings, so let's use something longer like $001$.
For example, the binary string $0011$ would be mapped to $01 \; 001 \; 01 \; 001 \; 10 \; 001 \; 10$.
Note that the only valid substring reversals are local to these pairs of bits.

\subsection{Substring Rotations}

\subsection{Middle-Levels?}

Middle levels with $n=2k+1$ == prefix-transpositions on $(k+1,k+1)$-combinations.

Middle levels has a global constraint.

\subsection{Kneser graph} : This has the same issue as the prefix reversal in strings.



%%% Subsection on de Bruijn sequences and 
\subsection{Polynomial-Time for De Bruijn Sequences and Universal Cycles}
\label{sec:back_deBruijn}

Our goal is to prove that various Gray code problems are (strongly) NP-Complete.
To motivate these results, it is helpful to note that many natural cases can be solved in polynomial-time.
For example, consider binary strings and the \emph{full-register shift} operations $\BITSHIFTS{n} = \{\shiftZeroSymbol,\shiftOneSymbol\}$ which shift a new bit into a binary string $b_1 b_2 b_3 \cdots b_n \in \BINARY{n}$ as follows,
\begin{equation*}
    \shiftZero{b_1 b_2 b_3 \cdots b_n} = b_2 b_3 \cdots b_n 0  \text{ and }  \shiftOne{b_1 b_2 b_3 \cdots b_n} = b_2 b_3 \cdots b_n 1.
\end{equation*}
Cyclic Gray codes that use these operations correspond to \emph{de Bruijn sequences}, which are cyclic sequences of length $2^n$ in which every member of $\BINARY{n}$ appears exactly once as a substring; see \cite{de1946combinatorial,de1975acknowledgement}
For example, $00010111$ is a de Bruijn sequence of order $n=3$;
the last $n-1$ substrings---$110$ and $100$---wrap-around.
We can generate all of its substrings, starting from the last non-wrapping substring---$111$--by applying the following full-register shifts   
\begin{equation} \label{eq:shiftSequence}
    111\ \shiftZeroSymbol\ 110\ \shiftZeroSymbol\ 100\ \shiftZeroSymbol\ 000\ \shiftOneSymbol\ 001\ \shiftZeroSymbol\ 010\ \shiftOneSymbol\ 101\ \shiftOneSymbol\ 011 \shiftOneSymbol.
\end{equation}
Note that flip list in \eqref{eq:shiftSequence} follows the bits in the de Bruijn sequence.
De Bruijn sequences have many interesting applications \cite{ngo2022entropy} and can be generated efficiently for all $n$ in many ways.
They are also characterized as the labels of Eulerian circuits in the well-known de Bruijn graph .

todo: mention relationship to linear feedback shift registers ... \cite{golomb2017shift}

De Bruijn sequences also exist and can be generated efficiently for various subsets of binary strings.
For example, the term \emph{weight} (or \emph{density}) describes the number of $1$s in a binary string, and sequences have been investigated for continuous range of weights; see \cite{ruskey2012bruijn} and \cite{stevens2014coolest}.
In particular, $001011$ is a de Bruijn sequence of order $n=3$ for strings with weight $1$ or $2$.
More generally, if $S \subseteq \BINARY{n}$ is a subset of $n$-bit binary strings, then the existence of a de Bruijn sequence for $S$ is equivalent to the decision problem $\GrayI[\BINARY{n},\BITSHIFTS{n}]{S}$.
These problems can be solved in polynomial-time by constructing the appropriate graph%
\footnote{For each $b_1 b_2 \ldots b_n \in S$ create node $b_1 b_2 \ldots b_{n-1}$ and an outgoing edge labeled $b_n$ to node $b_2 \ldots b_{n-1} b_n$.}
and checking if it is Eulerian.
Analogous results hold when binary strings are replaced by $k$-ary strings; see \cite{van1987circuits}.

De Bruijn sequences do not exist for permutations in one-line notation (e.g., $\PERMUTE{3} = \{123,132,213,231,312,321\}$).
However, they do exist if the substrings that are packed together omit the last redundant symbol (e.g., $\SHORT{3} = \{12,13,21,23,31,32\}$).
For example, $123132$ is a \emph{shorthand universal cycle}%
\footnote{Not to be confused with \emph{order isomorphic universal cycles for permutations} \cite{chung1992universal} \cite{johnson2009universal}.} 
for $n=3$, where the substring $31$ is shorthand for $312$, and it is followed by $13$ which is shorthand for $132$; see \cite{ruskey2010explicit} \cite{holroyd2012shorthand}.
In this setting, successive permutations (after the omitted final symbol is added) differ by $\ROTATEUNI{n} = \{\rotateZeroSymbol,\rotateOneSymbol\}$ which perform rotations on $p_1 p_2 p_3 \cdots p_n \in \PERMUTE{n}$ as follows,
\begin{equation*}
    \rotateZero{p_1 p_2 p_3 \cdots p_{n-1} p_n} = p_2 p_3 \cdots p_{n-1} p_n p_1  \text{ and }  \rotateOne{p_1 p_2 p_3 \cdots p_{n-1} p_n} = p_2 p_3 \cdots p_{n-1} p_1 p_n.
\end{equation*}
If $S \subseteq \PERMUTE{n}$, then the existence of a shorthand universal cycle for $S$ is equivalent to the decision problem $\GrayI[\PERMUTE{n},\ROTATEUNI{n}]{S}$.
By similar arguments, these problems can be solved in polynomial-time.
Moreover, the same is true when permutations are generalized to multiset permutations; see \cite{sawada2021universal,sawada2022constructing} and \cite{williams2009shift}.


%%% Outtakes from writing the new intro with induced subgraph reductions

This idea can be pushed even further by finding large cube graphs within a variety of other notable flip graphs.
This includes the \emph{permutohedron} $\PermGraph{n}$ whose vertices are the $n!$ permutations of $[n] = \{1,2,\ldots,n\}$ in one-line notation, with edges between those that differ in an \emph{adjacent-transposition} (or \emph{swap}).

Aaron: This section will explain the theory behind the results more carefully and include some specific results. 
two examples first is easier
second involves encoding sizes and connectivity are important

need to say how induced subgraphs are encoded in general

define induces for graph families
define polytime induces
wait, maybe don't need family notion at all.
just say one set induces another.
i.e., the set of cubes induces the set of grids
then the set of cubes poly-time induces the set of connected grids

when trying to establish hardness it may not be necessary to induce to entire graph family
for example, for Hamilton path only need connected
so connected grids polytime induce to (connected) cubes.
(in some cases we only get polytime if we induce to tighter set)

Let $\graph{G}_n$ be a family of graphs that is polytime inducible to a family of graphs $\graph{H}_n$.
cubes are inducible to grids?
grids is hard and we want to say that cubes is hard
this would normally be a reduction from grids to cubes
so we want to say induction from grids to cubes
but it's the opposite in the sense that we have induced subgraphs of the cube being grids

suppose that cubes induce grids.
that means that for every grid you can create a isomorphic induced subgraph of the cube in polytime.
if the problem is hard for induced subgraphs of the grid, then it will be hard for induced subgraphs of the cube.


so 
If
is a family of graphs
    If a decision problem is NP-hard for the induced subgraphs of a given family of graphs, 

Suppose that a decision problem is NP-hard for a set of graphs $\graphSet{G}$ that is closed under induced subgraphs (e.g., all grid graphs).
uh oh, we can't use this definition if we are restricted to connected grid graphs


yoyoyo you need to assume that $\graphClass{H}$ is somehow implicit to the decision problem...
perhaps define HamPath relative to a graph class...
then the input is the subset of vertices?
does the input also need to include reference to the specific graph in the set?
this is a problem with grid graphs as there are two parameters.
but perhaps only one that puts the points in standard position.
perhaps we need to say that the vertex set uniquely determines the underlying graph in the set?


filtering by connectivity...
Let $\mathbb{Z}_n = \{0, 1, \ldots, n-1\}$.
A set of points $S \subseteq \mathbb{Z}_r \times \mathbb{Z}_c$ is in \emph{standard position} if the minimum row and column coordinates are $0$, and the maximum row and column coordinates are $r-1$ and $c-1$, respectively.
The number of points in $S$ is denoted $|S|$.




more broadly, general theorem

theorem: 
induced subgraphs

these theorems do not imply hardness for special cases.
for example, hamilton paths of cube, middle levels, permutohedron, etc.

given a family of graphs parameterized by n, we say that polysize inducable if gi hi and write gi <p hi

graphic of grid <p cube <p permutohedron


0000
1000
1100
1110
1111
there are n+1

1000
1100
0100
0110
0010
0011
0001
there are 2n-1

100
110
010
011
001


%%% A chopped up version of inducements section ...
%%% I should have saved this before moving material to the appendix, oh well

\subsection{Polynomial-Time Inducement for NP-Hardness}
\label{sec:theory_poly}

To use inducement in hardness proofs, we need to compute containing graphs efficiently.
Before stating our notion of efficient, it is important address one subtlety.
When applying our notion of inducement from Definition \ref{def:induces}, we are able to consider full graphs and not their induced subgraphs, since the former implies the latter.
For example, the fact that hypercubes induce rectangular grid graphs implies that cubicals induce grid graphs.
We cannot take this simplified view when efficiency is a concern.
This is because efficiently computing an isomorphism for an induced subgraph cannot always be done by first computing the isomorphism for the full graph and then creating the appropriate induced subgraph of it.
%More specifically, this is an issue if the size of the induced subgraph is not a polynomially bounded by the size of the full graph.

To formalize our definition of efficiency, we say that a set of graphs is \emph{inducement closed} if every induced subgraph of a graph in the set is also in the set.
Similarly, the \emph{inducement closure} of a set of graphs is obtained by adding every induced subgraph to the set.
For example, the inducement closure of the set hypercube graphs is the set of cubical graphs.

\begin{definition} \label{def:polytimeInduces}
Let $\graphClass{H}$ be a family of graphs, and $\graphClass{H'}$ be its inducement closure.
A set of graphs $\graphClass{G}$ \emph{polynomial-time induces} $\graphClass{H}$ if $\graphClass{G}$ induces $\graphClass{H}$, and there a function $f$ that produces the induced subgraph, i.e., $f(\graph{H'}) = \graph{G}$ in polynomial-time relative to the encoding size of $\graph{H} \in \graphClass{H'}$.
\end{definition}

This definition leads to the following theorem.
We refer to the act of applying this theorem as a \emph{polynomial-time induced subgraph reduction}.

\begin{theorem} \label{thm:general}
Let $\graphClass{G}$ be a set of graphs that polynomial-time induces a set of graphs $\graphClass{H}$.
If a decision problem is NP-hard for the induced subgraphs of $\graphClass{H}$, then it is NP-hard for the induced subgraphs of $\graphClass{G}$.
\end{theorem}
\begin{proof}
TODO?
\end{proof}

Now we state the main result of this section.
A partial proof is provided here, with additional details in the appendix.
% When applying this theorem, one can use full graphs as opposed to their induced subgraphs.

Aaron: check that this theorem can refer to the full graphs and not the induced subgraphs
(i.e., hypercubes instead of cubicals, etc.).

\begin{theorem} \label{thm:three}
If a family of graphs $\graphClass{G}$ is polynomial-time inducible to rectangular grid graphs, hypercubes, or permutohedron, then the Hamilton path problem is NP-hard for the induced subgraphs of $\graphClass{G}$. 
\end{theorem}
\begin{proof}
The result is already known for rectangular grid graphs.
This is because the Hamilton path is NP-hard for grid graphs (i.e., the induced subgraphs of rectangular grid graphs) and that our definition polynomial-time inducement (see Definition \ref{def:polytimeInduces}) requires efficient mappings to the induced subgraphs.

The remainder of the proof involves two steps:
reducing hypercubes to grids, and reducing permutohedron to hypercubes.
Lemma \ref{lem:induces} already established inducement for these two steps, and we now need to establish that they can be performed efficiently.

The inducement from permutohedron to hypercubes in Lemma \ref{lem:induces} is a polynomial-time inducement.
This is because each $n$-bit binary string (requiring $O(n)$-bits to encode) can be converted to a permutation of $[2n]$ (requiring $O(n log(n))$-bit to encode) in polynomial-time.

The inducement from hypercubdes to grids in Lemma \ref{lem:induces} is not always a polynomial-time inducement.
However, it is when we restrict ourselves to grid graphs that are connected.
In other words, to efficiently reduce a Hamilton path problem on a grid graph to a Hamilton path problem on a cubical graph, we need to first test (in polynomial-time) if the grid graph is connected.
\begin{itemize}
    \item If the grid graph is not connected, then it does not have a Hamilton path.
    \item If the grid graph is connected, then we map it (in polynomial-time) to an isomorphic cubical graph.
\end{itemize}
The technical details involving connectivity and encoding sizes are further discussed in the appendix.
\end{proof}

.
.
.


\begin{theorem} \label{thm:connected}
Let $\graphClass{H}$ and $\graphClass{G}$ be families of graphs, and $\graphClass{H'}$ and $\graphClass{G'}$ be their inducement closures, respectively.
In addition, let $\graphClass{H''} \subseteq \graphClass{H'}$ be the connected graphs in $\graphClass{H'}$.
If the Hamilton Path problem is NP-hard for $\graphClass{H'}$ and $\graphClass{G}$ polynomial-time induces $\graphClass{H''}$, the then Hamilton Path problem is NP-hard for~$\graphClass{G'}$.
\end{theorem}
\begin{proof}
TODO
\end{proof}


\begin{lemma} \label{lem:connected}
Let $S \subseteq \mathbb{Z}_r \times \mathbb{Z}_c$ be a set of points in standard position.
If the induced subgraph of the grid graph $\GridGraph{r}{c}[S]$ is connected, then $S$ contains at least $r+c-1$ points.
That is, $|S| \geq r+c-1$.
\end{lemma}
\begin{proof}
Since $S$ is in standard position, a Hamilton path must use at least $r-1$ vertical edges to span each row, and $c-1$ horizontal edges to span each column.
A path with at least $r+c-2$ edges has at least $r+c-1$ vertices.
\end{proof}

Make some transitivity observation in Remark \ref{rem:inducedTransitive}...

\begin{remark} \label{rem:inducedTransitive}
    If graph $G$ is an induced subgraph of $H$, and $H$ is an induced subgraph of $I$, then .
    Moreover, if polytime, then polytime ...
\end{remark}

now conclude that HamPath is hard on hypercubes and permutohedron
i.e., prove Theorems from intro
